TREET: TRansfer Entropy Estimation via Transformers

Transfer entropy (TE) is an information theoretic measure that reveals the directional flow of information between processes, providing valuable insights for a wide range of real-world applications. This work proposes Transfer Entropy Estimation via Transformers (TREET), a novel attention-based approach for estimating TE for stationary processes. The proposed approach employs Donsker-Varadhan representation to TE and leverages the attention mechanism for the task of neural estimation. We propose a detailed theoretical and empirical study of the TREET, comparing it to existing methods on a dedicated estimation benchmark. To increase its applicability, we design an estimated TE optimization scheme that is motivated by the functional representation lemma, and use it to estimate the capacity of communication channels with memory, which is a canonical optimization problem in information theory. We further demonstrate how an optimized TREET can be used to estimate underlying densities, providing experimental results. Finally, we apply TREET to feature analysis of patients with Apnea, demonstrating its applicability to real-world physiological data. Our work, applied with state-of-the-art deep learning methods, opens a new door for communication problems which are yet to be solved.

==> Figures/TENE_DATA_benchmark.tex <==
%         GT
% -3 0.829244694517248
% -2 0.811474676368
% -1 0.698623737745733
% 0 0.415182801705413
% 1 0.131741865665092
% 2 0.0188909270428257
% 3 0.0011209088935776
\newcommand{\GT}[1]{%
    \ifnum#1=-3 0.829\fi%
    \ifnum#1=-2 0.811\fi%
    \ifnum#1=-1 0.699\fi%
    \ifnum#1=0 0.415\fi%
    \ifnum#1=1 0.132\fi%
    \ifnum#1=2 0.019\fi%
    \ifnum#1=3 0.001\fi%
}

% \addtolength{\tabcolsep}{-6pt}    
% \begin{table}[t]
% \centering
% \caption{
% TE estimation extended benchmark 
% }
% \resizebox{
% 0.48\textwidth
% % 1\textwidth
% }{!}{%
    \begin{tabular}{cc|ccccccc}
        \toprule
        $\lambda$ &  & \textbf{-3} & \textbf{-2} & \textbf{-1} & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} \\ 
        \midrule
        % \textbf{Ground} & \\ 
        % \textbf{Truth}
        % \backslashbox{GT}{Model}

        \multicolumn{2}{c|}{\diaghead{\theadfont Ground Ground Truth}%
        {Model, $l$}{Ground$\quad$\\Truth$\quad$}}
        % \diaghead{\theadfont Ground Truth Truth}%
        % {Model, $l$}{Ground\\Truth} &  
        & \GT{-3} & \GT{-2} & \GT{-1} & \GT{0} & \GT{1} & \GT{2} & \GT{3} \\ 
        \midrule
        \multirow{8}{*}{$\quad$\textbf{\rotatebox[origin=c]{90}{TREET}}} 
        & $1$  & \diffColor{0.812}{\GT{-3}} & \diffColor{0.792}{\GT{-2}} & \diffColor{0.667}{\GT{-1}} & \diffColor{0.395}{\GT{0}} & \diffColor{0.126}{\GT{1}} & \diffColor{0.016}{\GT{2}} & \diffColor{-0.000}{\GT{3}} \\ 
        & $2$  & \diffColor{0.826}{\GT{-3}} & \diffColor{0.796}{\GT{-2}} & \diffColor{0.681}{\GT{-1}} & \diffColor{0.392}{\GT{0}} & \diffColor{0.117}{\GT{1}} & \diffColor{0.014}{\GT{2}} & \diffColor{0.000}{\GT{3}} \\ 
        & $4$  & \diffColor{0.825}{\GT{-3}} & \diffColor{0.798}{\GT{-2}} & \diffColor{0.682}{\GT{-1}} & \diffColor{0.393}{\GT{0}} & \diffColor{0.115}{\GT{1}} & \diffColor{0.013}{\GT{2}} & \diffColor{0.000}{\GT{3}} \\ 
        & $7$  & \diffColor{0.820}{\GT{-3}} & \diffColor{0.799}{\GT{-2}} & \diffColor{0.679}{\GT{-1}} & \diffColor{0.405}{\GT{0}} & \diffColor{0.121}{\GT{1}} & \diffColor{0.015}{\GT{2}} & \diffColor{0.001}{\GT{3}} \\  
        & $9$  & \diffColor{0.815}{\GT{-3}} & \diffColor{0.802}{\GT{-2}} & \diffColor{0.686}{\GT{-1}} & \diffColor{0.403}{\GT{0}} & \diffColor{0.126}{\GT{1}} & \diffColor{0.017}{\GT{2}} & \diffColor{0.001}{\GT{3}} \\ 
        & $19$ & \diffColor{0.824}{\GT{-3}} & \diffColor{0.805}{\GT{-2}} & \diffColor{0.690}{\GT{-1}} & \diffColor{0.405}{\GT{0}} & \diffColor{0.128}{\GT{1}} & \diffColor{0.017}{\GT{2}} & \diffColor{0.001}{\GT{3}} \\ 
        & $49$ & \diffColor{0.829}{\GT{-3}} & \diffColor{0.811}{\GT{-2}} & \diffColor{0.694}{\GT{-1}} & \diffColor{0.409}{\GT{0}} & \diffColor{0.128}{\GT{1}} & \diffColor{0.018}{\GT{2}} & \diffColor{0.001}{\GT{3}} \\ 
        & $99$ & \diffColor{0.829}{\GT{-3}} & \diffColor{0.810}{\GT{-2}} & \diffColor{0.693}{\GT{-1}} & \diffColor{0.410}{\GT{0}} & \diffColor{0.115}{\GT{1}} & \diffColor{0.017}{\GT{2}} & \diffColor{0.001}{\GT{3}} \\ 
        \midrule
        \multirow{8}{*}{$\quad$\textbf{\rotatebox[origin=c]{90}{TENE}}} 
        & $1$  & \diffColor{0.823}{\GT{-3}} & \diffColor{0.807}{\GT{-2}} & \diffColor{0.696}{\GT{-1}} & \diffColor{0.416}{\GT{0}} & \diffColor{0.126}{\GT{1}} & \diffColor{0.014}{\GT{2}} & \diffColor{0.000}{\GT{3}} \\ 
        & $2$  & \diffColor{0.814}{\GT{-3}} & \diffColor{0.782}{\GT{-2}} & \diffColor{0.688}{\GT{-1}} & \diffColor{0.390}{\GT{0}} & \diffColor{0.115}{\GT{1}} & \diffColor{0.013}{\GT{2}} & \diffColor{0.000}{\GT{3}} \\ 
        & $4$  & \diffColor{0.430}{\GT{-3}} & \diffColor{0.760}{\GT{-2}} & \diffColor{0.602}{\GT{-1}} & \diffColor{0.382}{\GT{0}} & \diffColor{0.119}{\GT{1}} & \diffColor{0.013}{\GT{2}} & \diffColor{-0.001}{\GT{3}} \\ 
        & $7$  & \diffColor{999}{\GT{-3}} & \diffColor{999}{\GT{-2}} & \diffColor{0.698}{\GT{-1}} & \diffColor{0.354}{\GT{0}} & \diffColor{0.090}{\GT{1}} & \diffColor{0.013}{\GT{2}} & \diffColor{-0.000}{\GT{3}} \\  
        & $9$  & \diffColor{999}{\GT{-3}} & \diffColor{999}{\GT{-2}} & \diffColor{524.551}{\GT{-1}} & \diffColor{0.359}{\GT{0}} & \diffColor{0.091}{\GT{1}} & \diffColor{0.014}{\GT{2}} & \diffColor{-0.000}{\GT{3}} \\ 
        & $19$ & \diffColor{999}{\GT{-3}} & \diffColor{999}{\GT{-2}} & \diffColor{999}{\GT{-1}} & \diffColor{1.796}{\GT{0}} & \diffColor{0.038}{\GT{1}} & \diffColor{0.021}{\GT{2}} & \diffColor{0.000}{\GT{3}} \\ 
        & $49$ & \diffColor{-999}{\GT{-3}} & \diffColor{-999}{\GT{-2}} & \diffColor{-999}{\GT{-1}} & \diffColor{999}{\GT{0}} & \diffColor{0.027}{\GT{1}} & \diffColor{0.010}{\GT{2}} & \diffColor{-0.002}{\GT{3}} \\ 
        & $99$ & \diffColor{999}{\GT{-3}} & \diffColor{999}{\GT{-2}} & \diffColor{999}{\GT{-1}} & \diffColor{999}{\GT{0}} & \diffColor{0.102}{\GT{1}} & \diffColor{-0.002}{\GT{2}} & \diffColor{-0.002}{\GT{3}} \\ 
        \midrule
        \multirow{8}{*}{$\quad$\textbf{\rotatebox[origin=c]{90}{Copnet}}}  
        & $1$  & \diffColor{0.835}{\GT{-3}} & \diffColor{0.810}{\GT{-2}} & \diffColor{0.688}{\GT{-1}} & \diffColor{0.397}{\GT{0}} & \diffColor{0.111}{\GT{1}} & \diffColor{-0.000}{\GT{2}} & \diffColor{-0.022}{\GT{3}} \\ 
        & $2$  & \diffColor{0.819}{\GT{-3}} & \diffColor{0.786}{\GT{-2}} & \diffColor{0.676}{\GT{-1}} & \diffColor{0.377}{\GT{0}} & \diffColor{0.106}{\GT{1}} & \diffColor{-0.004}{\GT{2}} & \diffColor{-0.017}{\GT{3}} \\ 
        & $4$  & \diffColor{0.900}{\GT{-3}} & \diffColor{0.864}{\GT{-2}} & \diffColor{0.747}{\GT{-1}} & \diffColor{0.469}{\GT{0}} & \diffColor{0.193}{\GT{1}} & \diffColor{0.087}{\GT{2}} & \diffColor{0.079}{\GT{3}} \\ 
        & $7$  & \diffColor{1.297}{\GT{-3}} & \diffColor{1.268}{\GT{-2}} & \diffColor{1.135}{\GT{-1}} & \diffColor{0.903}{\GT{0}} & \diffColor{0.649}{\GT{1}} & \diffColor{0.571}{\GT{2}} & \diffColor{0.575}{\GT{3}} \\  
        & $9$  & \diffColor{1.703}{\GT{-3}} & \diffColor{1.679}{\GT{-2}} & \diffColor{1.558}{\GT{-1}} & \diffColor{1.357}{\GT{0}} & \diffColor{1.106}{\GT{1}} & \diffColor{1.054}{\GT{2}} & \diffColor{1.053}{\GT{3}} \\ 
        & $19$ & \diffColor{4.862}{\GT{-3}} & \diffColor{4.834}{\GT{-2}} & \diffColor{4.750}{\GT{-1}} & \diffColor{4.574}{\GT{0}} & \diffColor{4.431}{\GT{1}} & \diffColor{4.428}{\GT{2}} & \diffColor{4.432}{\GT{3}} \\ 
        & $49$ & \diffColor{17.958}{\GT{-3}} & \diffColor{17.936}{\GT{-2}} & \diffColor{17.859}{\GT{-1}} & \diffColor{17.779}{\GT{0}} & \diffColor{17.622}{\GT{1}} & \diffColor{17.669}{\GT{2}} & \diffColor{17.687}{\GT{3}} \\ 
        & $99$ & \diffColor{43.625}{\GT{-3}} & \diffColor{43.572}{\GT{-2}} & \diffColor{43.547}{\GT{-1}} & \diffColor{43.421}{\GT{0}} & \diffColor{43.356}{\GT{1}} & \diffColor{43.445}{\GT{2}} & \diffColor{43.442}{\GT{3}} \\ 

        \bottomrule
        \multicolumn{9}{p{\benchmarkrowlen}}{
            Comparing \treetext{}, TENE and Copnet. 
            The process is given by \eqref{eq:tenedata_flipping_process} and the true TE can be calculated for varying $\lambda$ \cite{zhang2019itene}. 
            The color intensity signifies the extent of deviation from the ground truth.
            The value is constant for any order - $l \geq 1$ since $\sTE(l) = \sTE(1)$.
            Our proposed benchmark is an extended version of the one presented in \cite{zhang2019itene} to include variable length input to calculate different orders of TE.
            In the given benchmark, $\rho$ is set to 0.9, while the $\lambda$ and $l$ parameters are varied.
        }    
    \end{tabular}%
% }

% \label{tab:te_benchmark}
% \end{table}
% \addtolength{\tabcolsep}{6pt}    


